Warm-up Free Policy Optimization: Improved Regret in Linear Markov Decision Processes

Policy Optimization (PO) methods are among the most popular Reinforcement Learning (RL) algorithms in practice. Recently, Sherman et al. [2023a] proposed a PO-based algorithm with rate-optimal regret guarantees under the linear Markov Decision Process (MDP) model. However, their algorithm relies on a costly pure exploration warm-up phase that is hard to implement in practice. This paper eliminates this undesired warm-up phase, replacing it with a simple and efficient contraction mechanism. Our PO algorithm achieves rate-optimal regret with improved dependence on the other parameters of the problem (horizon and function approximation dimension) in two fundamental settings: adversarial losses with full-information feedback and stochastic losses with bandit feedback.

==> Defs/mathdefs.tex <==
%%Requeiried packages and preliminary definitions, needed by the options
\RequirePackage{mathtools}
% \RequirePackage{thmtools}
% \RequirePackage{amsfonts}
\RequirePackage{dsfont}
\RequirePackage{delimset}

%%Body of the package, most of the declarations appear here.

% Parenthethis
% \newcommand{\prn}[1]{\left( #1 \right)}
% \newcommand{\prn}[2][*]{\brk#1{#2}}
% \newcommand{\brc}[1]{\left\lbrace #1 \right\rbrace}
% \newcommand{\brc}[2][*]{\brk[c]#1{#2}}
% \newcommand{\brk}[1]{\left\lbrack #1 \right\rbrack}
% \newcommand{\abs}[1]{\left| #1 \right|}
% \newcommand{\underbracetxt}[2]{\underset{#2}{\underbrace{#1}}}

% Functions
% \newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
% \newcommand{\innProd}[2]{\langle #1,#2 \rangle}
\newcommand{\innProd}[2][*]{\brk[a]#1{#2}}
\newcommand{\ceil}[2][*]{\delim\lceil\rceil#1{#2}}
\newcommand{\floor}[2][*]{\delim\lfloor\rfloor#1{#2}}
\newcommand{\indEvent}[2][*]{\mathds{1}_{\brk[c]#1{#2}}}
% \newcommand{\indEvent}[2][*]{\mathbb{1}{\brk[c]#1{#2}}}
\newcommand{\indFunc}[2][\infty]{\mathds{I}_{\brk[s]{#2,#1}}}
\newcommand{\indFuncAt}[3][\infty]{\indFunc[#1]{#2}\brk*{#3}}
\newcommand{\tr}[2][*]{\mathrm{Tr}\brk*{#2}}
\newcommand{\overbar}[1]{\mkern 2mu\overline{\mkern-2mu#1\mkern-2mu}\mkern 2mu}
\newcommand{\tran}{^{\mkern-1.5mu\mathsf{T}}}


% Standard Math Notations
\newcommand{\Oof}[2][*]{O\brk#1{#2}}
\newcommand{\OtildeOf}[2][*]{\smash{\widetilde{O}}\brk#1{#2}}
\newcommand{\EE}[1][]{\mathbb{E}_{#1}}
\newcommand{\PR}[1][]{\mathbb{P}_{#1}}
\newcommand{\EEBrk}[2][*]{\EE\delim{[}{]}#1{#2}}
\newcommand{\RR}[1][]{\mathbb{R}^{#1}}
\newcommand{\ZZ}[1][]{\mathbb{Z}^{#1}}
\newcommand{\ZZplus}[1][]{\mathbb{Z}^{#1}_{+}}
\newcommand{\PP}[2][*]{\mathbb{P}\brk#1{#2}}

\newcommand{\sphere}[1]{\mathcal{S}^{#1}}
\newcommand{\ball}[1]{\mathcal{B}^{#1}}

% Probability
\newcommand{\gaussDist}[2]{\mathcal{N}\brk0{#1, #2}}

% Math operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}

% Definitions
\DeclarePairedDelimiterX\setDef[1]\lbrace\rbrace{\def\given{\;\delimsize\vert\;}#1}
\newcommand{\seqDef}[3]{\brk[c]*{#1}_{#2}^{#3}}

% General
\def\noi{\noindent}

\newcommand{\ifrac}[2]{#1/#2}
\newcommand{\minEigOf}[2][*]{\lambda_{\mathrm{min}}\brk#1{#2}}
\newcommand{\maxEigOf}[2][*]{\lambda_{\mathrm{max}}\brk#1{#2}}


\newcommand{\rootT}{\ensuremath{\smash{\sqrt{T}}}\xspace}

\newcommand{\clip}{\mathrm{clip}}
